SolefulTap: Augmenting Tap Dancing Experience using a Floor-Type Impact Display

We propose SolefulTap for a novel tap dancing experience. It allows users to feel as if they are tap dancing or appreciate a tap dancing performance using the sensations of their own feet. SolefulTap uses a method called Step Augmentation that provides audio-haptic feedback to users, generating impacts in response to users' simple step motions. Our prototype uses a floor-type impact display consisting of pressure sensors, which detect users' steps, and solenoids, which generate feedback through impact. Through a preliminary user study, we confirmed that the system can provide untrained users with the experience of tap dancing. This study serves as a case study that provides insight into how a reactive environment can affect the human capabilities of physical expression and the sensation experienced.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}
We proposed SolefulTap, which provides a novel tap dancing experience through Step Augmentation using a floor-type impact display.
Step Augmentation is achieved by providing audio-haptic feedback to users in response to their steps.
The feedback is generated by impacting the floor surface with a set of solenoids.

We explored user interactions and experiences created by the system through prototype demonstrations, representing application scenarios.
After each demonstration, a user survey was conducted using a questionnaire, and verbal feedback was received.
As a result, we confirmed that the system was able to provide untrained users with the experience of tap dancing.
Given the findings, we discussed the design of impact patterns and the scalability of the system as well as the future prospects of applying the proposed system.

SolefulTap represents an approach to human augmentation that focuses on the interaction between human bodies and environments, specifically the soles and floor.
Despite not wearing any device on the user’s body, our approach provides a physical expression that feels as if the user is performing a tap dance based on reactions from the environment.
Our study, therefore, is an exploration of novel forms of physical expression through interactions with a reactive environment.
We hope that our viewpoint will help diversify the approaches toward building human capabilities in the field of human augmentation.

==> sections/relatedwork.tex <==
\section{Related Work}
\label{sec:RelatedWork}
We provide a novel tap dancing experience by applying Step Augmentation in the interaction between the soles and floor.
Here, we introduce previous studies focusing on the soles interfaces and on the floor interfaces, respectively, and describe the position of our research.

% \subsection{Performance Augmentation}
% \label{sec:PerformanceAugmentation}
% One of the most common extensions of dance expression is stage direction using music and lighting.
% By altering the sound and light to match the dancer's movements, it emphasizes the performer's movements and creates a scene that the viewer finds impressive.
% In the research using advanced technologies, the dancers' expression will be evaluated using a system that utilizes wearable technology such as footwear~\cite{Paradiso:2000}, full body LED display~\cite{Izuta:2019}, AR technology~\cite{Clay:2012} and VR technology~\cite{Konno:2016}. 
% All of these research examples require a suit or electronic device to be attached to the dancer's body, and only audiovisual information is fed back to the dancer.
% In this research, we try to extend the expression without depending on the dancer's outfit by placing sensors and actuators only in the environment.
% In this research, we try to expand the expression of the dancer's body by placing sensors and actuators only on the environment side.

\subsection{Sole Interface}
\label{sec:SoleInterface}
In general, sole interfaces have been researched as part of developing footwear-type devices, which have been studied as a wearable computer technology.
Although various input modalities have been studied for footwear devices, relatively few studies have been conducted for output modalities regardless of the advantage of being able to use the sensation of soles~\cite{Don:2021}. 
For example, in studies focusing on haptic presentation to the soles, devices have been developed that provide vibration stimulation~\cite{Tachiquin:2021,Sakai:2018}, inclination~\cite{31:CabBoots}, and temperature~\cite{63:ShoeSoleSense}. 
However, footwear-type devices have physical restrictions such as a relatively small space where sensors and actuators can be placed, and the weight of a device inhibits users' movements.
Paradiso et al.'s pioneering study using a footwear-type device in dance performance also focused solely on sensing technology~\cite{Paradiso:2000}.
If we consider haptic feedback to soles in contact with the floor, the restrictions mentioned above can be mitigated by placing the actuator on the floor side.

\subsection{Floor Interface}
\label{sec:FloorInterface}
Floor interfaces have been studied as environment-embedded interfaces by installing sensors and actuators on the floor. 
As the advantage of this approach, users do not have to attach a device to the body.
Floor interfaces are often used for sensing in smart home systems such as for fall detection~\cite{Feng:2016} and position estimation~\cite{Li:2018} in our daily lives. 
Actuation is often used to improve the immersion and presence of the experience. 
For example, a system that generates large-scale vibrations exists for use in amusement attractions~\cite{Disney_patent} because there are less restrictions on the device size. 
Law et al.~\cite{Law:2008} and Visell et al.~\cite{Visell:2010} have studied floor interactions where the user's input and the output of the system spatiotemporally coincide~(I/O coincidence).
Regarding tap dance, Shibasaki et al. studied a system using the floor~\cite{Shibasaki:2016}, which was applied as an interface for the hearing impaired to appreciate a performance through haptic sensation. 
The system measures the tap sounds made by the dancers using microphones and conveys haptic information in a single direction to the audience through the floor device.

In this study, we used audio-haptic feedback to form a user's interaction with other users and the environment. 
By using a floor interface that has both sensing and actuation functions to enable Step Augmentation, described in Section~\ref{sec:concept}, SolefulTap provides a novel tap dancing experience without restricting the body motions of the users.
